Sterile Neutrinos from Dark Matter: A $\nu$ Nightmare?

We provide a comprehensive study of observable spectra from dark matter pair-annihilation or decay into sterile (right-handed) neutrinos. This occurs, for instance, in neutrino portal dark matter models, where a sterile neutrino acts as the portal between dark matter and the Standard Model sector. The subsequent decays of right-handed neutrinos produce detectable Standard Model particles, notably photons, positrons, and neutrinos. We study the phenomenology of models where the right-handed neutrino masses are below the GeV scale, as well as models where they are at, or significantly heavier than, the TeV scale. In both instances, and for different reasons, the standard tools, including Monte Carlo simulations, are both inadequate and inaccurate. We present the complete framework to compute the relevant branching ratios for right-handed neutrino decays and the spectra of secondary photons, positrons, and neutrinos for a broad range of dark matter and right-handed neutrino masses. We discuss the general features of such signals, and compare the spectra to standard signals from dark matter annihilation/decay into bottom quarks. Additionally, we provide open source code1 that can be used to compute such spectra. The code is available at https://github.com/LoganAMorrison/blackthorn.

==> settings/enviornments.tex <==
\newenvironment{myalg}{%      define a custom environment
	\bigskip\noindent%         create a vertical offset to previous material
	\refstepcounter{myalgctr}% increment the environment's counter
	\textsc{Algorithm \themyalgctr}% or \textbf, \textit, ...
	\newline%
}{\par\bigskip}  %          create a vertical offset to following material
\numberwithin{myalgctr}{section}

==> settings/newcommands.tex <==
%Shortcuts
\newcommand{\vr}{\pmb{\scriptr}}
\renewcommand{\r}{\scriptr}
\newcommand{\hr}{\;\h{\!\r}}
\newcommand{\rs}{\scriptr^{\; 2}}
\renewcommand{\v}[1]{\vec{#1}}
\newcommand{\ol}[1]{\overline{#1}}
\renewcommand{\b}[1]{{\bf #1}}
\newcommand{\delmu}{\partial^{\mu}}
\newcommand{\delmd}{\partial_{\mu}}
\newcommand{\phis}{\phi^*}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\diag}{\text{diag}}
\renewcommand*{\Rnfont}{\scshape}
\newcommand{\anticomm}[2]{\{#1,#2\}}
\newcommand{\spp}[2]{\left(#1 \cdot #2\right)}

%Common QFT symbols
\newcommand{\sla}[1]{\cancel{#1}} %Feynman slash
\newcommand{\vRel}{v_{\text{rel}}} %v_rel
\newcommand{\dPiLips}{d\Pi_{\text{LIPS}}} %d Pi_LIPS
\newcommand{\mGam}{m_{\gamma}} %d Pi_LIPS
\newcommand{\pd}[1]{\partial_{#1}}


==> settings/packages.tex <==
%Misc (forgot what these are for)
\def\mathclap#1{\text{\hbox to 0pt{\hss$\mathsurround=0pt#1$\hss}}}
\usepackage[makeroom]{cancel}
\usepackage{xcolor}
\newcommand\Ccancel[2][black]{\renewcommand\CancelColor{\color{#1}}\cancel{#2}}
\usepackage[parfill]{parskip}


%Math packages 
\usepackage{amsmath,amssymb,amsthm,amsfonts,verbatim,enumerate,graphicx}


%Physics Packages 
\usepackage{physics}
\usepackage{tensor}
\usepackage{siunitx}
\usepackage{circuitikz}


%Feynman Diagrams
\usepackage{tikz-feynman}



%Figures 
\usepackage{graphics}
\usepackage{caption}
\usepackage{subcaption}
\usepackage{epstopdf}
\usepackage[utf8]{inputenc} % set input encoding (not needed with XeLaTeX)
\usepackage{pgfplots}


%Tikz figures
\usepackage{tikz} %for making pretty figures
\usepackage[tikz]{bclogo}
\usepackage{tikz-3dplot}
\tdplotsetmaincoords{60}{110}
\usetikzlibrary{fadings}
\usetikzlibrary{arrows,shapes,positioning}
\usetikzlibrary{decorations.markings}
\tikzstyle arrowstyle=[scale=1]
\tikzstyle directed=[postaction={decorate,decoration={markings,
		mark=at position .5 with {\arrow[arrowstyle]{stealth}}}}]
\tikzstyle reverse directed=[postaction={decorate,decoration={markings,
		mark=at position .5 with {\arrowreversed[arrowstyle]{stealth};}}}]
\tikzstyle photon = [decorate, decoration={snake}]


%Bibtex
\usepackage{biblatex}



%Particle masses 
\newcommand{\mnp}{m_{\pi^0}}     %%Neutral pion 
\newcommand{\mcp}{m_{\pi^{\pm}}} %%Charged pion 
\newcommand{\mchi}{m_{\chi}}	 %%DM


\usepackage[toc,page]{appendix}
\usepackage{todonotes}

% needed for creating hyperlinks in the document, the option colorlinks=true gets rid of the awful boxes, breaklinks breaks lonkg links (list of figures)
\usepackage[colorlinks=true,breaklinks]{hyperref} 


%Modify the section titles
\usepackage[explicit]{titlesec}
%\titleformat{\section}{\normalfont\Large\bfseries}{}{0em}{#1\ \thesection}


==> settings/pagesetup.tex <==
%Stuff for title
\makeatletter % Need for anything that contains an @ command
\newcommand{\horrule}[1]{\rule{\linewidth}{#1}}
\renewcommand{\maketitle} % Redefine maketitle to conserve space
{ \begingroup \vskip 10pt
	\begin{center}
		\horrule{5pt}
		\huge {\bf \@title}
		\vskip 10pt
		\large{\@author}
		\vskip 10pt
		\large{\@date}  \end{center}
	\horrule{5pt} \\[0.4cm]
	\vskip 10pt \endgroup \setcounter{footnote}{0} }

%Edit page size
\usepackage{geometry}
\geometry{
	top=1 in,
	inner=1 in,
	outer=1 in,
	bottom=1 in,
	headheight=1ex,
	headsep=3ex
}

%Header
\usepackage{changepage}
\usepackage{fancyhdr}
\setlength{\headheight}{15pt}
\pagestyle{fancyplain}
\usepackage{lastpage}
%\renewcommand{\sectionmark}[1]{\markright{#1}{}}
\makeatletter
%\renewcommand\@seccntformat[1]{}
\makeatother
\lhead{L. A. Morrison}
\chead{5D - HW 2}
\rhead{Page \thepage\ / \pageref{LastPage}}
\renewcommand{\headrulewidth}{0.4pt}
\fancyfoot[C]{}

